Emotionalism within People-Oriented Software Design

In designing most software applications, much effort is placed upon the functional goals, which make a software system useful. However, the failure to consider emotional goals, which make a software system pleasurable to use, can result in disappointment and system rejection even if utilitarian goals are well implemented. Although several studies have emphasized the importance of people's emotional goals in developing software, there is little advice on how to address these goals in the software system development process. This paper proposes a theoretically-sound and practical method by combining the theories and techniques of software engineering, requirements engineering, and decision making. The outcome of this study is the Emotional Goal Systematic Analysis Technique (EG-SAT), which facilitates the process of finding software system capabilities to address emotional goals in software design. EG-SAT is easy to learn and easy to use technique that helps analysts to gain insights into how to address people's emotional goals. To demonstrate the method in use, a two-part evaluation is conducted. First, EG-SAT is used to analyze the emotional goals of potential users of a mobile learning application that provides information about low carbon living for tradespeople and professionals in the building industry in Australia. The results of using EG-SAT in this case study are compared with a professionally-developed baseline. Second, we ran a semi-controlled experiment in which 12 participants were asked to apply EG-SAT and another technique on part of our case study. The outcomes show that EG-SAT helped participants to both analyse emotional goals and gain valuable insights about the functional and non-functional goals for addressing people's emotional goals.

==> note.tex <==

Questionnaires etc (page 22 footnotes) are not shared


Table 4 is a bit confusing; maybe a comparative matrix? How were repetitive goals measured?









==> tables/EG-SATsummary.tex <==
\begin{landscape}


\begin{table}[]
\centering
\caption{Summary of EQ-FAST Analysis in \emph{Building Quality Passport} Case Study}
\label{emotionalconcerns}

%\resizebox{\textwidth}{!}{%
%\footnotesize
\scriptsize
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Emotional (Sub-emotional) Goal}  & \textbf{Proposed Quality Goals} & \textbf{Proposed Functional Goals} & \textbf{Comment} \\
\toprule
Freedom and Flexibility & Repeatability, Modularity, Flexible & $-$ & $-$ \\
(Sense of learning at my own pace) \\ (In control) \\
\hline
Sense of time efficiency  & Short and Sharp, Easy to understand, \\  & Reusable Contents, Compatibility / Integrity   &  $-$ & $-$ \\
\hline
Sense of trust in information & Accurate Content, Reliable Platform & $-$ & $-$ \\
\hline
Sense of reality & $-$ & Simulation, Case-based learning & $-$\\
\hline
Knowledgeable \& Skillful & Tangible  & $-$ & Refer to " Sense of reality" \\
\hline
Professional & $-$ & Represent Experiences and Skills, Represent & Refer to "Sense of networking"  \\ &  & Certificates and Qualifications, Like and Follow, & \& "Connected"   \\ && Represent Badges \& Rewards, Represent  \\ && Progress, Networking  \\
\hline
Qualified & $-$ & Represent Experiences and Skills, Represent & Refer to "Sense of networking"  \\ && Certificates \& Qualifications, Like \& Follow,  & \& "Connected" \\ &&  Represent Badges \& Rewards, Represent \\ && Progress, Networking  & \\ 
\hline
Connected & $-$ & Networking & $-$\\
\hline
Supported and assisted  & Easy to find, Instant & Resource, Instructor Feedback & Refer to "Sense of Networking" \\ &&& \& "Connected"\\
\hline
Self-confident & & like and follow & Refer to "Sense of Achievement  \\

(Sense of contribution)&&& and Success",  "Connected",    \\
(Prepared)&&& "Sense of Networking",  \\&&& "Supported and Assisted" \\&&& "Professional" and " Qualified"  \\

\hline
Sense of opportunity  & $-$ & Estimator (Current position, market  \\&& demand, wealth generation) & $-$
 \\
\hline
Sense of monetary (wealth)  & $-$ & $-$ & Refer to "Sense of Networking"  \\ &&&  \& "Connected", \\ &&& "Professional" \& "Qualified" \\
\hline
Sense of achievement \& success & & Benchmarking, Assessment/ Grading,  & Refer to "Professional" \&  \\ (Sense of ongoing learning)&& Goal Planning, Makes progress visible 
(Progressive) & "Qualified" \\
(Sense of completion) && Credentialing Acknowledgement,  \\   &  & Offer Badges \& Reward  \\

\hline
Sense of networking & $-$ & Networking \& Peer Feedback & $-$ \\
\hline
Sense of cost-effectiveness  & Reusable Contents  &  $-$ &  $-$ \\
 \hline
Sense of promotion \& progression   & $-$ & Make progress visible, Benchmarking, Assessment/ & Refer to "Professional" \& \\ &&Grading, Credentialing Acknowledgement, & "Qualified" \\ && Offer Badges and Reward \\
\hline
Sense of being cutting edge & $-$ & Track \& Trace Technology News, Technology & Refer to "Professional" \&  \\ && Statistics and history of use & "Qualified"

 \\
\hline
%In control & $-$ & Flexible  &    $-$  &    $-$  \\
%\hline
Sense of fun & $-$ & Gamification  &  $-$\\
\hline
Sense of competition  &  $-$ & Make progress visible, Benchmarking, Assessment/ & Refer to "Sense of Fun" \\ &&Grading, Credentialing Acknowledgement, \\ && Offer Badges and Reward &    \\

\bottomrule
\end{tabular}% 
%}
\end{table}
\end{landscape}






==> tables/compare.tex <==
\begin{table}[ht]
\centering
\small
%\footnotesize
%\scriptsize
\caption{The Comparison of the Results in Using PCA and PEAF Approaches}
\label{compare}
%\end{table}
%\begin{table}
%\centering

%\footnotesize
%%\scriptsize
%\caption{The Comparison of the Results in Using PCA and UEAF Approaches}
%\label{compare}
\begin{tabular}{lrr} 
\toprule
Count & PCA & PEAF\\
\midrule
Emotional goals & 12 & 20 \\
Emotional codes & 44 & 117 \\ 
\midrule
Ideal self & 13 & 69 \\
Public self & 7 & 50 \\ 
Affiliation & 7 & 36 \\
Social pleasure & 41 & 101 \\
Ideological pleasure & 4 & 10 \\
Physical pleasure & 0 & 0 \\
Memories & 0 & 0 \\ \midrule
Self-expression & 20 & 119 \\
Affiliation & 7 & 36 \\
Memories & 0 & 0 \\
Pleasure & 45 & 111 \\
 \bottomrule
\end{tabular}
\end{table}


==> tables/definition.tex <==
%\tm{I have re-formatted the table to user `default' latex formatting. Hard-coding line breaks etc., makes it much more difficult to re-used later (requires formatting when the page sizes change etc)}

\begin{table}[!h]
\centering
\small
%\scriptsize
\caption{Themes and Drivers Definitions}
\label{definition}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lp{0.6\textwidth}l}
\toprule
\textbf{Themes \textbackslash Drivers} & \textbf{Definition} & \textbf{Source(s)} \\ \midrule
\textbf{Self-expression} & The people's interest to feel a distinct personal identity from others through expressing the personal identity such as feelings, thoughts or ideas & \cite {mugge2008product, Collins, ball1992role, kleine1995possession} \\
~~$\bullet$ Ideal-self & The people's interest to feel like a person they would imagine to be & \cite {sirgy1982self} \\
~~$\bullet$ Public-self & The people's interest regarding the image they would like others have of them & \cite {sirgy1982self} \\ \midrule
\textbf{Affiliation} & The people's interest to feel a sense of relationship with others and  belonging to social groups & \cite{champoux2016organizational, kleine1995possession} \\ \midrule
\textbf{Memories} & The people's interest to feel a sense of the past, happy moments,  people, occasions and places that are important for them & \cite {klein2012memory, csikszentmihalyi1981meaning} \\ \midrule
\textbf{Pleasure} & The people's interest to feel happy satisfaction and enjoymen & \cite {Mugge, jordan2002designing, maclachlan2009exploring, maclachlan2009let} \\[1mm] 
~~$\bullet$ Physical pleasure & The people's interest to feel pleasure due to experiencing sensory perception (five senses) & \cite {jordan2002designing} \\ 
~~$\bullet$ Social pleasure & The people's interest to feel pleasure due to having social interaction or better social status/image & \cite {jordan2002designing} \\
~~$\bullet$ Ideological pleasure & The people's interest to feel pleasure due to dealing with their values and beliefs & \cite {jordan2002designing} \\ \bottomrule
\end{tabular}
% %}
\end{table}


==> tables/efficiency.tex <==
\begin {comment}
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Efficiency Analysis Results}
\label{tab:efficiency}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll|lllll|lllll|lllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{4}{*}{\textbf{Technique}}} & \multicolumn{21}{c}{\textbf{Metric}} \\ \cmidrule(l){2-22} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ave. Time\\ (Minutes)\end{tabular}}}}  & \multicolumn{5}{c}{\textbf{Perceived ease of learn}} & \multicolumn{5}{c}{\textbf{Perceived ease of use}} & \multicolumn{5}{c}{\textbf{Perceived usefulness}} & \multicolumn{5}{c}{\textbf{Intention to use}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{5}{c}{(out of five)} & \multicolumn{5}{c}{(out of five)} & \multicolumn{5}{c}{(out of five)} & \multicolumn{5}{c}{(out of five)} \\


 \cline{2-22} 
 \\

%& & $--$ & $-$ & $0$ & $+$ & $++$ & $--$ & $-$ & $0$ & $+$ & $++$ & $--$ & $-$ & $0$ & $+$ & $++$ & $--$ & $-$ & $0$ & $+$ & $++$\\

 %\hline
 
1 &  &  &  &  &  &  & &  &  &  &   &  &  &  &  &  &  &  &  &  &  \\
2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
3 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
4 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
5 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
6 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
7 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
8 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
9 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
10 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
11 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
12 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
13 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
14 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 

\bottomrule

%\multicolumn{22}{l}{* $--$ Strongly disagree $~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$  $++$ Strongly agree} 

\end{tabular}% 
}

\end{table}

\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Efficiency Analysis Results}
\label{tab:efficiency}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\toprule
\multicolumn{1}{l}{\multirow{4}{*}{\textbf{Technique}}} & \multicolumn{4}{c}{\textbf{Metric}} \\ \cline{2-5} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Perceived \\ ease of learn \\ (out of five)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Perceived \\ ease of use \\ (out of five)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Perceived \\ usefulness\\ (out of five)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Intention \\ to use\\ (out of five)\end{tabular}}} \\ 
\toprule
POSE &  &  &  &  \\ 
Synectics &  &  &  &  \\ 
Barinstorming &  &  &  &  \\ 
SCAMPER &  &  &  &  \\ 
Attribute Listing &  &  &  &  \\
EG-SAT &  &  &  &  \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/evaluation.tex <==
\begin{table}[t!]
\centering
\footnotesize
%\scriptsize
\caption{Qualitative Questions}
\label{tab:evaluation}
\begin{tabular}{@{}llllll|lllll@{}}
\toprule
\multirow{2}{*}{} %& %\multicolumn{10}{c}{Metric} \\
 
 {\multirow{2}{*}{\textbf{ID}}}   & \multicolumn{5}{c|}{\textbf{Completeness}} & \multicolumn{5}{c}{\textbf{Correctness}} \\
% \midrule
 & \multicolumn{5}{c|}{Distribution *} & \multicolumn{5}{c}{Distribution *} \\
 \cline{2-11} 
 & $--$ & $-$ & $0$ & $+$ & $++$ & $--$ & $-$ & $0$ & $+$ & $++$\\
 \hline

IS1  &  &  &  &  &  &  &  &  &  &  \\
IS2 &  &  &  &  &  &  &  &  &  &  \\
IS3 &  &  &  &  &  &  &  &  &  &  \\
IS4 &  &  &  &  &  &  &  &  &  &  \\
IS5 &  &  &  &  &  &  &  &  &  &  \\
%IS6 &  &  &  &  &  &  &  &  &  &  \\
IS6 &  &  &  &  &  &  &  &  &  &  \\
IS7 &  &  &  &  &  &  &  &  &  &  \\
IS8 &  &  &  &  &  &  &  &  &  &  \\
%IS9 &  &  &  &  &  &  &  &  &  &  \\
PS1 &  &  &  &  &  &  &  &  &  &  \\
PS2 &  &  &  &  &  &  &  &  &  &  \\
AF1 &  &  &  &  &  &  &  &  &  &  \\
AF2 &  &  &  &  &  &  &  &  &  &  \\
SP1 &  &  &  &  &  &  &  &  &  &  \\
Sp2 &  &  &  &  &  &  &  &  &  &  \\
SP3 &  &  &  &  &  &  &  &  &  &  \\
IP1 &  &  &  &  &  &  &  &  &  &  \\
IP2 &  &  &  &  &  &  &  &  &  &  \\
IP3 &  &  &  &  &  &  &  &  &  &  \\
IP4 &  &  &  &  &  &  &  &  &  &  \\
IP5 &  &  &  &  &  &  &  &  &  &  \\
IP6 &  &  &  &  &  &  &  &  &  &  \\
PP1 &  &  &  &  &  &  &  &  &  &  \\
PP2 &  &  &  &  &  &  &  &  &  &  \\

\bottomrule

\multicolumn{11}{c}{* $--$ Strongly disagree $~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$  $++$ Strongly agree} 
\end{tabular}
\end{table}

==> tables/negativetopositive.tex <==
\begin{table*}[!h]
\centering
%\scriptsize
%\footnotesize
\caption{Some samples of converting negative emotional concerns  to positive emotional goals}
\label{negativetopositive}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\textbf{Emotional Concerns} & \textbf{Emotional Goals} \\ \hline
having cloudy mind & Having a sense of good feeling \\ \hline
Lack of People's Trust on me & Having a sense of being trusted \\ \hline
Lack of People's Respect on me & Having a sense of being respected \\ \hline
personal stress and anxiety & Having a sense of calm \\ \hline
Lack of  clarity and stability & Having a sense of receiving clear, simple and accurate information \\ \hline
People's reluctance  for support and assistance & Having a sense of support and assistance \\ \hline
Lack of privacy & Having a sense of privacy \\ \hline
Having a sense of misleading & Having a sense of receiving clear and accurate information \\ \hline
Hopelessness & Having a sense of motivation and hopefulness \\ \hline
Having a sense of misleading & Having a sense of receiving clear and accurate information \\ \hline
losing self esteem & Having a sense of self-respect and self-worth \\ \hline
Lake of empathy & Having a s sense of being empathized with and listened to. \\ \hline
Hopelessness & Having a sense of motivation and hopefulness \\ \hline
\end{tabular}%
}
\end{table*}


==> tables/oldtables.tex <==
\begin{table}[H]
\small
\centering
\caption{Goal-Driver Profile for `Sense of being in Control'}
\label{gdpSIC}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Having a Sense of In Control}}\\ Total Emotional Concerns: 1
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 0 \\
Affiliation & 0 \\
Social Pleasure & 0 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Empowered'}
\label{gdpSOE}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Having a Sense of Empowered}}\\ Total Emotional Concerns: 3
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 0 \\
Affiliation & 0 \\
Social Pleasure & 67 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Connected'}
\label{gdpSOC}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Connected}}\\ Total Emotional Concerns: 13
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 100 \\
Affiliation & 92 \\
Social Pleasure & 100 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Clarity and Trust of Information'}
\label{gdpSOCT}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Clarity and Trust}}\\ Total Emotional Concerns: 15
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 0 \\
Public Self & 0 \\
Affiliation & 40 \\
Social Pleasure & 100 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Self-Worth'}
\label{gdpSOS}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Self-worth}}\\ Total Emotional Concerns: 5
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 60 \\
Public Self & 100 \\
Affiliation & 0 \\
Social Pleasure & 20 \\
Ideological Pleasure & 100 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}

==> tables/qualitative.tex <==
\begin{table}[!t]
\centering

%\small
\caption{Qualitative Questions}
\label{tab:qualitative}
\footnotesize
\begin{tabular}{p{1.75cm}p{2cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}}
\hline

\multicolumn{1}{c}{\multirow{2}{*}{Property}} & \multicolumn{1}{c}{\multirow{2}{*}{Indices}} & \multicolumn{5}{c}{Distribution} \\ \cline{3-7} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $--$ & $-$ & $\circ$ & $+$ & $++$ 

\\ \hline

 \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Usability \&\\  Usefulness\end{tabular}} & Consistency &  &  &  & 1 &  \\  
 & Completeness &  &  &  & 1 &  \\  
 & Correctness &  &  &  & 1 &  \\ 
 & Tracability &  &  &  & 1 &  \\ 
 & Clarity &  &  &  &  & 1 \\  
 & \begin{tabular}[c]{@{}l@{}}Share \\ Understanding\end{tabular} &  &  & 1 &  &  
 
 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} Output \\ Validity \end{tabular}} & Consistency &  &  &  &  & 1 \\  
 & Completeness &  &  &  & 1 &  \\ 
 & Correctness &  &  &  &  & 1 \\ \hline
 
\end{tabular}
\end{table}


==> tables/questions.tex <==
\begin{table*}[]
\centering
\caption{The related question for each emotional attachment driver}
\label{questions}
%\scriptsize
%\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|}
\hline
\textbf{Driver} & \textbf{Question} \\ \hline
Ideal Self & How this system can help me to become a person I would like to be in terms of ...  \\ \hline
Public Self & How this system can help me to create the image that  I would like other people \\ 
& have of me in terms of `a person with / who ...'  \\ \hline
Affiliation  & How this system can help me to belong to a group? \\ \hline
Social Pleasure & How this system can help me to improve my social pleasure in terms of `better social\\ 
& interaction,  better social status ...' \\ \hline
Ideological Pleasure & To what extent this system is aligned with  / respects / considers my values and \\ 
& beliefs in terms of ...  \\ \hline
Physical Pleasure & How this system can help me to feel sense of   realism in terms of ... (Sight, Hearing, Taste,  \\ & Smell 
 and Touch)"   \\ \hline
Memories & How this system can help me to remind positive memories
in terms of `something  on the \\ 
& past,  specific occasion, person, nostalgia ,...'  \\ \hline
\end{tabular}%
}
\rachel{This table is a key part of the process you undertook when extending desmets model. I would put this in the same text where you explain what each driver is. It acts as a description of how each emotional concern translates into a technology setting.}
\end{table*}


==> tables/sum1.tex <==
\begin{table}
    \centering
    \caption{Summary of emotional attachment drivers}
\label{sum1}
\small

\begin{tabular}{lrrrrrrrr} 

\toprule
\textbf{} & 
\textbf{\rotatebox[origin=c]{90}{Ideal Self}}& 
\textbf{\rotatebox[origin=c]{90}{Public Self}}& 
\textbf{\rotatebox[origin=c]{90}{Affiliation}}& 
\textbf{\rotatebox[origin=c]{90}{Social Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Ideological Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Physical Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Memories}}
& \textbf{Sum}\\
\midrule
\textbf{Self-expression} & 10 & 2 &  &  &  &  &  & \textbf{12} \\
\textbf{Affiliation} &  &  & 2 &  &  &  &  & \textbf{2} \\ 
\textbf{Memories} &  &  &  &  &  &  & 0 & \textbf{0} \\
\textbf{Pleasure} &  &  &  & 3 & 6 & 2 &  & \textbf{11}\\

\bottomrule
\end{tabular}
\end{table}


==> tables/sum2.tex <==
\begin{table}
\centering
\caption{Summary of emotional attachment drivers for each theme - PEAF approach }
\label{sum2}


\small

\begin{tabular}{lrrrrrrrr} 

\toprule
\textbf{} & 
\textbf{\rotatebox[origin=c]{90}{Ideal Self}}& 
\textbf{\rotatebox[origin=c]{90}{Public Self}}& 
\textbf{\rotatebox[origin=c]{90}{Affiliation}}& 
\textbf{\rotatebox[origin=c]{90}{Social Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Ideological Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Physical Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Memories}}
& \textbf{Sum}\\
\midrule
\textbf{Self-expression} & 69 & 50 &  &  &  &  &  & \textbf{119} \\
\textbf{Affiliation} &  &  & 36 &  &  &  &  & \textbf{36} \\ 
\textbf{Memories}  &  &  &  &  &  &  & 0 & \textbf{0} \\
\textbf{Pleasure} &  &  &  & 101 & 10 & 0 &  & \textbf{111}\\

\bottomrule
\end{tabular}
\end{table}

